Low-Resource Cross-Lingual Adaptive Training for Nigerian Pidgin

Developing effective spoken language processing systems for low-resource languages poses several challenges due to the lack of parallel data and limited resources for fine-tuning models. In this work, we target on improving upon both text classification and translation of Nigerian Pidgin (Naija) by collecting a large-scale parallel English-Pidgin corpus and further propose a framework of cross-lingual adaptive training that includes both continual and task adaptive training so as to adapt a base pre-trained model to low-resource languages. Our studies show that English pre-trained language models serve as a stronger prior than multilingual language models on English-Pidgin tasks with up to 2.38 BLEU improvements; and demonstrate that augmenting orthographic data and using task adaptive training with back-translation can have a significant impact on model performance.

==> tables/011_machine_translation_word_based.tex <==
\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cc}
\textbf{Word Tokenization} & \textbf{Bible+JW300} & \textbf{JW300} \\
\midrule
EN to PCM  & 23.87 & 17.73          \\
PCM to EN  & 22.61 & 24.67          \\ 
\midrule
\end{tabular}}
\caption{ \small Machine Translation 4-4 Layers, 10 heads, 300 embeddings 1200 FFNN}
\label{tab:biblejw300 wordbased}
\end{table}

==> tables/012_domain_information_tables.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccc}

\hline
\textbf{Domain} & \textbf{Classification Task}              & \textbf{Label Type} & \textbf{Train}                                                                                 & \textbf{Dev}                                                                                & \textbf{Test} & \textbf{Classes} \\ \hline
PCM & Multi Class  & Sentiment Anaylsis  & \begin{tabular}[c]{@{}c@{}}negative    4497\\ positive    2091\\ neutral      131\end{tabular} & \begin{tabular}[c]{@{}c@{}}negative    338\\ positive    278\\ neutral      63\end{tabular} & \begin{tabular}[c]{@{}c@{}}negative    665\\ positive    514\\ neutral     117\end{tabular} & 3                \\ \hline
PCM Clean & Multi Class  & Sentiment Anaylsis  & \begin{tabular}[c]{@{}c@{}}negative    4497\\ positive    2091\\ neutral      130\end{tabular} & \begin{tabular}[c]{@{}c@{}}negative    338\\ positive    278\\ neutral      5\end{tabular} & \begin{tabular}[c]{@{}c@{}}negative    665\\ positive    514\\ neutral     6\end{tabular} & 3                \\ \hline
\end{tabular}}
\caption{PCM classification dataset}
\end{table*}

==> tables/013_pcm_classification_examples.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{ll}
\hline
PCM Classification Example                                                  & Label    \\ \hline
make e see wetin hin fine face and stature dey cause for my marital house o & Positive \\ \hline
as in the word strong ehn so tey e fit break padlock,                       & negative \\ \hline
see as e be like person wey don baff with dulux white oil paint             & neutral  \\ \hline
\end{tabular}
\caption{PCM Classification examples}
\end{table*}

==> tables/014_parrellel_dataset_similiarity.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{|cccc|}
\hline
\multicolumn{4}{|c|}{\textbf{Percentage PCM/English in the different datasets}}                                                                             \\ \hline
\multicolumn{1}{|c|}{Bible"PCM"}   & \multicolumn{1}{c|}{0.238}              & \multicolumn{1}{c|}{0.339}               & 0.177                  \\ \hline
\multicolumn{1}{|c|}{JW300 "PCM"}    & \multicolumn{1}{c|}{0.0656}             & \multicolumn{1}{c|}{0.303}               & 0.1321                 \\ \hline
\multicolumn{1}{|c|}{TreeBank "PCM"} & \multicolumn{1}{c|}{0.1130}             & \multicolumn{1}{c|}{0.16}                & 0.526                  \\ \hline
\multicolumn{1}{|c|}{PCM/EN}      & \multicolumn{1}{c|}{Bible"EN"} & \multicolumn{1}{c|}{JW300 "EN"} & TreeBank "EN" \\ \hline
\end{tabular}
\caption{Cross-Lingual Similarity between English to PCM accross different resources}
\label{tab:Cross-Lingual Similarity}
\end{table*}

==> tables/015_pretraining_corpus.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Percentage PCM/English in the different datasets} & \textbf{Pretrainign Corpus}                                      & \textbf{\#Tokens}  & \textbf{\#unique Tokens} \\ \hline
\textbf{AFRI-BERT}                                        & \cite{Afri-BERT}                                 & 9,516,579 & 164,056         \\ \hline
Enrich                                           & \cite{ajisafe2020towards}               & 136,292   & 9,588           \\ \hline
BBC PCM monolingual                              & \href{https://www.bbc.com/pidgin}{BBC Pidgin} & 1,889,551 & 76,557          \\ \hline
\textbf{UNMT}                                             & \cite{lent2021language}                        & 1,328,121          & \textbf{47,582}          \\ \hline
\end{tabular}}
\caption{Cross Lingual Language Modelling Pre-training Corpus}
\label{tab:pretraining_corups}
\end{table*}

==> tables/017_crosslingual_pretraining.tex <==
\begin{table}[]
\begin{tabular}{|c|c|l|}
\hline
\textbf{Cross-lingual Domain data set} & \textbf{Number of Lines} & F1Score \\ \hline
Afri-BERT (Common Crawal and BBC news) &                          &         \\ \hline
BBC                                    &                          &         \\ \hline
Religous (Bible \& JW300)              &                          &         \\ \hline
Twitter (Naija Senit)                  &                          &         \\ \hline
NSC  Tree bank                         &                          &         \\ \hline
\end{tabular}
\end{table}

==> tables/018_cross_lingual_domain_adaptation.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Cross-lingual Domain data set} & \textbf{Number of Lines} \\ \hline
Afri-BERT (Common Crawal and BBC news) & 176,843                      \\ \hline
BBC                                    & 4,148                      \\ \hline
Religous (Bible \& JW300)              & 52,058                       \\ \hline
Twitter (Naija Senit)                  & 8,524                       \\ \hline
NSC  Tree bank                         & 9,240                       \\ \hline
\end{tabular}
\caption{The Datasets and their domains}
\label{tab: cross-domain adaptation}
\end{table*}

==> tables/019_cross_domain_LM_pretrain.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Model} & \textbf{Lines} & \textbf{F1} \\ \hline
AfriBERT data  & 176,843        & .729        \\ \hline
BBC data       & 4,148          & .792        \\ \hline
Religious      & 52,058         & .770        \\ \hline
Naija Senti    & 9,524          & .797        \\ \hline
Treebank       & 9,249          &             \\ \hline
En-PLM++       &                & .\textbf{825}        \\ \hline
RoBerta-En     &                & .801       \\ \hline
\end{tabular}
\caption{cross lingual pretraining}
\label{tab:cross-lingual pretraining results}
\end{table*}

==> tables/01_examples_from_the_datasets.tex <==

\begin{table*}[]
\begin{tabular}{lp{6.3cm}p{6.3cm}}
\hline
Source & English   & Pidgin    \\ \hline
Bible  & And Saul, hearing that David had gone to Gath, went after him no longer. & Wen Saul hear sey David don run go Gat, e kon stop to porshu am. \\
JW300  & Keep peace with one another.                                             & Make una be people wey like peace.                               \\
NSC Treebank & You had electricity in your area last night?                             & Una get light for una area last night?       \\  
Naijasenti & -- & make e see wetin hin fine face and stature dey cause for my marital house o \\
BBC Pidgin & -- & Peter Obi joins Labour Party: Di former Anambra state govnor confam im defection for Twitter \\
IWSLT'15 & rainforest in pursuit of data on a key molecule & -- \\
       \hline
\end{tabular}
\label{tab:dataexampless}
\caption{Examples from the datasets}

\end{table*}


==> tables/020_synthetic_data_.tex <==
\begin{table*}[]
\begin{tabular}{|c|c|c|}
\hline
        & \textbf{English-PCM} & \textbf{PCM-EN} \\ \hline
T5-Base & 29.519               & 25.26           \\ \hline
\end{tabular}
\caption{Synthetic}
\label{tab:senthetic data}
\end{table*}

==> tables/02_orthographic_variation_the_word_bacause.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lllll} \hline
             & because & bikos & cause & cos \\ \hline
Bible        & 265     & 1,108 & -   & -     \\
JW300 & X     &      &    &     \\ 
USC Treebank & 243     & -     & 7   & 3    \\ 
%BBC & X     &      &    &     \\ 
\hline
\end{tabular}
\caption{Orthographic variation of the word \textit{because}, along with raw counts per dataset.}\label{tab:variationbecause}
\end{table}

==> tables/04_back-translation_data.tex <==


\begin{table}[H]
\begin{tabular}{|l|ll|}
\hline
\cellcolor[HTML]{656565}       & \multicolumn{2}{l|}{\textbf{Back Translation Data}}     \\ \hline
\textbf{Synthetic source} & \multicolumn{1}{l|}{\textbf{English}} & \textbf{Pidgin} \\ \hline
\textbf{Number of Lines}       & \multicolumn{1}{l|}{133,167}           & 162,815          \\ \hline
\textbf{Traning Model}         & \multicolumn{1}{l|}{\textbf{PCM-EN}}  & \textbf{EN-PCM} \\ \hline
\end{tabular}
\caption{Back-Translation Data}
\end{table}








==> tables/05_en-plm++.tex <==


\begin{table}[H]
\centering
\begin{tabular}{cccc}
\hline
\cellcolor[HTML]{343434} & \multicolumn{3}{c}{Weighted F1 Score}                                                     \\ \hline
Epoch                    & \multicolumn{1}{c}{EN-PLM ++}                     & \multicolumn{1}{c}{EN-PLM} & PCM-PLM \\ \hline
48                       & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}0.813} & \multicolumn{1}{c}{0.786}  &         \\ \hline
                         & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}}      & \multicolumn{1}{c}{}       &         \\ \hline
                         & \multicolumn{1}{c}{}                              & \multicolumn{1}{c}{}       &         \\ \hline
\end{tabular}
\caption{En-PLM++ means more pretraining for RoBERTa-EN model, on the collected PCM data. EN-PLM RoBERTa En model without more pretraining. PCM-PLM RoBERTa model pretrained only on the PCM data from Scratch }
\end{table}

==> tables/06_back_translation_results_b+_wbt.tex <==


\begin{table}[H]
\begin{tabular}{|c|cc|cc|}
\hline
                               & \multicolumn{2}{c|}{\textbf{EN(Tgt)}}                  & \multicolumn{2}{c|}{\textbf{PCM(Tgt)}}                 \\ \cline{2-5} 
\multirow{-2}{*}{\textbf{BPE}} & \multicolumn{1}{c|}{\textbf{B+}}     & \textbf{WBT}  & \multicolumn{1}{c|}{\textbf{B+}}    & \textbf{WBT}   \\ \hline
\textbf{EN (Src)}                    & \multicolumn{2}{c|}{\cellcolor[HTML]{000000}\textbf{}} & \multicolumn{1}{c|}{\textbf{}}      & \textbf{24.29}   \\ \hline
\textbf{PCM (Src)}                   & \multicolumn{1}{c|}{\textbf{31.04}}  & \textbf{28.76}     & \multicolumn{2}{c|}{\cellcolor[HTML]{000000}\textbf{}} \\ \hline
\end{tabular}
\caption{Back Translation Results, B+ is model with back-translation. While WBT is a model without back-translation }
\end{table}

==> tables/08_old_tables_9_to_11.tex <==
% table 1
\begin{table}[H]
\begin{tabular}{|c|cc|cc|}
\hline
                      & \multicolumn{2}{c|}{EN (Tgt)}                                    & \multicolumn{2}{c|}{PCM (Tgt)}                                        \\ \cline{2-5} 
\multirow{-2}{*}{BPE} & \multicolumn{1}{c|}{B+}                 & JW300 & \multicolumn{1}{c|}{B+}                 & JW300 \\ \hline
EN (Src)      & \multicolumn{2}{c|}{\cellcolor[HTML]{343434}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}27.54} & 24.29    \\ \hline
PCM (Src)   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}25.56} & 13      & \multicolumn{2}{c|}{\cellcolor[HTML]{343434}}                   \\ \hline
\end{tabular}
\caption{\label{tab:table-name} 6-6 layers,  B+ "Bible + JW300", 4 heads, 4K vocab, 256 embeddings, BPE .}
\end{table}


% table 2 
\begin{table}[H]
\begin{tabular}{|c|cc|cc|}
\hline
                       & \multicolumn{2}{c|}{EN (Tgt)}                                    & \multicolumn{2}{c|}{PCM (Tgt)}                                        \\ \cline{2-5} 
\multirow{-2}{*}{Word} & \multicolumn{1}{c|}{B+}                 & JW300 & \multicolumn{1}{c|}{B+}                 & JW300 \\ \hline
EN (Src)       & \multicolumn{2}{c|}{\cellcolor[HTML]{343434}}                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}23.87} & 17.73      \\ \hline
 PCM (Src)    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}22.61} & 24.67      & \multicolumn{2}{c|}{\cellcolor[HTML]{343434}}                   \\ \hline
\end{tabular}
\caption{\label{tab:table-name}4-4 layers,  B+ "Bible + JW300", 10 heads,300 embeddigns, Word level tokenization.}

\end{table}

% table 3
\begin{table}[H]
\begin{tabular}{|c|cc|cc|}
\hline
                      & \multicolumn{2}{c|}{EN (Tgt)}                                     & \multicolumn{2}{c|}{PCM (Tgt)}                                         \\ \cline{2-5} 
\multirow{-2}{*}{BPE} & \multicolumn{1}{c|}{B+}                  & JW300 & \multicolumn{1}{c|}{B+}                  & JW300 \\ \hline
EN (Src)      & \multicolumn{2}{c|}{\cellcolor[HTML]{343434}}                    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}30.74*} & 24.29      \\ \hline
 PCM (Src)   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}28.76*} & 13      & \multicolumn{2}{c|}{\cellcolor[HTML]{343434}}                    \\ \hline
\end{tabular}
\label{tab:older_results} 
\caption{6-6 layers,  B+ "Bible + JW300" , 4 heads, 4K vocab, 256 embeddings, BPE, shared-embedding.}

\end{table}































==> tables/21_orthographicResuts.tex <==
\begin{table*}[ht]
\begin{tabular}{|c|c|c|}
\hline
\textbf{Model Type}                                                                                        & \textbf{EN-PCM} & \textbf{PCM-EN} \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}T5-En Base\\ "Bible+JW300+TreeBank"\end{tabular}}                       & 34.901          & 32.13           \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}T5-EN base\\ "Orthographic Data,\\ Bible,Jw300, TreeBank"\end{tabular}} & 35.154          & 32.897          \\ \hline
\end{tabular}
\caption{ \small T5-EN base model trained on English "JW300, Bible, Treebank" against "Orthographic Augmented data, JW300, Bible, TreeBank}
\label{tab:orthographic Variation results}
\end{table*}

==> tables/22_orthographicDataTestedonRealEnglish.tex <==
\begin{table*}[ht]
\begin{tabular}{|c|c|c|}
\hline
\textbf{Model Type}                                                                                        & \textbf{EN-PCM} & \textbf{PCM-EN} \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}T5-En Base\\ "Bible+JW300+TreeBank"\end{tabular}}                       & 36.165           & 33.22           \\ \hline
\textbf{\begin{tabular}[c]{@{}c@{}}T5-EN base\\ "Orthographic Data,\\ Bible,Jw300, TreeBank"\end{tabular}} & 36.04           & 33.79           \\ \hline
\end{tabular}
\caption{comparing T5-EN base model trained on both real synthetic data J300, Bible and Treebank against training on those data alongside the augmented data}
\label{tab:orthographicVariationTestonRealEnglish}
\end{table*}
